Measurements of $\pi^{\pm}$, $K^{\pm}$ and proton yields from the surface of the T2K replica target for incoming 31 GeV/c protons with the NA61/SHINE spectrometer at the CERN SPS

Measurements of the $\pi^{\pm}$, $K^{\pm}$, and proton double differential yields emitted from the surface of the 90-cm-long carbon target (T2K replica) were performed for the incoming 31 GeV/c protons with the NA61/SHINE spectrometer at the CERN SPS using data collected during 2010 run. The double differential $\pi^{\pm}$ yields were measured with increased precision compared to the previously published NA61/SHINE results, while the $K^{\pm}$ and proton yields were obtained for the first time. A strategy for dealing with the dependence of the results on the incoming proton beam profile is proposed. The purpose of these measurements is to reduce significantly the (anti)neutrino flux uncertainty in the T2K long-baseline neutrino experiment by constraining the production of (anti)neutrino ancestors coming from the T2K target.

==> Makefile <==
TEX = pdflatex
BIB = bibtex
#main file
texfile = na61_pT2KRT


FIGS=$(wildcard figures/*/*.*)
#all texfiles
#SECS=$(wildcard *.tex)

REVTEX:=$(CURDIR)/revtex4-1/tex/latex/revtex
REVBST:=$(CURDIR)/revtex4-1/bibtex/bst/revtex
NATBIB:=$(CURDIR)/natbib

export TEXINPUTS:=$(CURDIR):$(REVTEX):$(TEXINPUTS)
export BSTINPUTS:=$(CURDIR):$(REVBST):$(BSTINPUTS)


.PHONY: pdf
.PHONY: clean

all: pdf

pdf: $(texfile).pdf

paper: $(texfile).pdf

$(texfile).pdf : $(FIGS) na61_pT2KRT.bib
	$(TEX) $(texfile)
	$(BIB) $(texfile)
	$(TEX) $(texfile)
	$(TEX) $(texfile)
	$(TEX) $(texfile)
	

clean:
	@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}

revtex: 
	mktexlsr $(PWD)/revtex4-1

natbib: $(NATBIB)/natbib.sty

$(NATBIB)/natbib.sty:
	rm natbib.sty; cd $(NATBIB); ls; latex natbib.ins; cd ../; ln -s $(NATBIB)/natbib.sty .

